Prompting Large Language Models to Tackle the Full Software Development Lifecycle: A Case Study

Recent advancements in large language models (LLMs) have significantly enhanced their coding capabilities. However, existing benchmarks predominantly focused on simplified or isolated aspects of coding, such as single-file code generation or repository issue debugging, falling short of measuring the full spectrum of challenges raised by real-world programming activities. In this case study, we explore the performance of LLMs across the entire software development lifecycle with DevEval, encompassing stages including software design, environment setup, implementation, acceptance testing, and unit testing. DevEval features four programming languages, multiple domains, high-quality data collection, and carefully designed and verified metrics for each task. Empirical studies show that current LLMs, including GPT-4, fail to solve the challenges presented within DevEval. Our findings offer actionable insights for the future development of LLMs toward real-world programming applications.

==> src/baseline.tex <==


We introduce a baseline system formulated for our \devterm, building upon the foundations of ChatDev \cite{qian2023communicative, qian2023experiential}. 
ChatDev is a virtual, chat-powered software development system that adheres to the conventional waterfall model. 
It bifurcates the development process into four primary tasks (dubbed as phrases in ChatDev): design, coding, testing, and documentation. 
Within this system, multiple LLM agents assume diverse roles such as programmers, reviewers, and testers, pertinent to each phase. 
ChatDev is characterized by its utilization of a chat chain mechanism, which segments each phase into smaller, atomic tasks. 
This approach enables context-sensitive, multi-turn dialogues between two distinct roles, facilitating the proposal and validation of solutions for individual tasks.

In contrast to ChatDev, our development of baseline system incorporates several features and enhancements. 
We have restructured the task design to align closely with the evaluation criteria of \devterm. 
Specifically, this includes the integration of comprehensive input to the system, exemplified by well-structured PRDs. 
This integration is crucial in addressing and examining the issue of hallucination in controlled experimental settings. 
Moreover, our baseline system expands upon the capabilities of ChatDev, supporting a wider range of tasks, including standard Object-Oriented programming designs (UML class and sequence diagrams), repository planning (architecture design), environment setup, and acceptance testing.
A significant advancement in our baseline system is its compatibility with multiple programming languages and their corresponding runtime environments. 
This feature is coupled with the provision of comprehensive execution feedback to the system. 

==> src/dataset.tex <==

\begin{table}[]
\centering
\scalebox{0.6}{
\begin{tabular}{c|c|c|c|c}
\toprule
 & \textbf{Python} & \textbf{C/C++} & \textbf{Java} & \textbf{JavaScript$^\ddag$}  \\
\midrule
Domain$^{\dag}$ & \begin{tabular}[c]{@{}c@{}}\mytag{NLP}{c1}\mytag{CV}{c2}\\ \mytag{DL}{c3}\mytag{ALGO}{c4}\\ \mytag{API}{c5}\mytag{Tool}{c8}\end{tabular}  & \begin{tabular}[c]{@{}c@{}} \mytag{DB}{c6} \\ \mytag{ALGO}{c4}\\ \mytag{Tool}{c8}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\mytag{CV}{c2}\mytag{DB}{c6} \\ \mytag{ALGO}{c4} \\ \mytag{Tool}{c8} \end{tabular}  & \mytag{WEB}{c7}            \\
\midrule
\#Repo                                                         & 10     & 5     & 5    & 2          \\
\midrule
\begin{tabular}[c]{@{}c@{}}Avg. \\ \#Code File\end{tabular}    & 2.2    & 7.0   & 5.4  & 6.0        \\
\midrule
\begin{tabular}[c]{@{}c@{}}Avg. \\ \#Code Line\end{tabular}    & 276    & 495   & 524  & 617       \\
\midrule
\begin{tabular}[c]{@{}c@{}}Avg. \\ \#Accep. Tests\end{tabular} & 3.0    & 5.4   & 2.4  & 2        \\
\midrule
\begin{tabular}[c]{@{}c@{}}Avg. \\ \#Unit Tests\end{tabular}   & 12.4   & 11.8  & 8.2   & -           \\
\midrule
\begin{tabular}[c]{@{}c@{}}Avg. \\ Coverage \end{tabular}       & 91.8   & 95.0  & 64.9$^{\ast}$ & -  \\
\bottomrule      
\end{tabular}
}
\caption{\devterm~Statistics. ${\dagger}$: \devterm~covers a range of domains including NLP, computer vision, deep learning, algorithm implementation, API applications, Database applications, web service (both frontend and backend), and general tools and utilities. ${\ddagger}$: We do not include unit testing for JavaScript as checking functional correctness is not applicable to pure static web pages. Correctness of page rendering and user interaction handling is checked using acceptance tests. ${\ast}$: Interfaces with thirty-party libraries that are not used to implement the designated functionalities are not supplied with test cases, resulting in relatively lower overall test coverage. 
%$^\star$: Average test coverage achieved by accompanying reference unit tests.
}
\label{tab:repo stats}
\end{table}

\subsection{Dataset Construction}
% \label{sec:dataset construnction}

The data preparation process in our work consists of three distinct phases: repository preparation, code cleanup, and document preparation.

The initial phase, repository preparation, involves selecting high-quality, well-structured candidate repositories from a GitHub dump. 
Recognizing the impracticality of constructing a repository from scratch, we employed a filtering process to identify suitable candidates. 
Moreover, we imposed a constraint on the total number of lines of code to ensure the repositories' complexity remains manageable, facilitating the evaluation of current LLMs.

During the code cleanup phase, our postgraduate student annotators were tasked with setting up the required environment as stipulated in the repositories' README files.
 They then executed the code to verify its functionality.
 Following this sanity check, the annotators were instructed to meticulously refine the code repositories. 
 This refinement included the removal of unnecessary auxiliary files. 
 To ascertain code quality, the annotators were also required to run existing unit and acceptance tests, or to develop additional tests, ensuring they meet the standards of the oracle test and achieve satisfactory coverage.

The final phase, document preparation, involved the creation of standard software design documents, namely, UML class and sequence diagrams, and architecture designs, for each repository. 
We provide annotators with specific guidelines and templates for these documents. 
The annotators were responsible for ensuring that these design documents corresponds accurately and cohesively with the respective code repositories.

\subsection{Dataset Statistics}

In Table \ref{tab:repo stats}, we present an exhaustive statistical breakdown of our datasets.
\devterm~contains a collection of 22 curated repositories, spanning across four widely-used programming languages (Python, C/C++, Java, JavaScript) and a diverse range of domains.
The dataset is characterized by its multi-file structure.
The Python repositories in our dataset are relatively straightforward, with each repository comprising approximately two files and an average of 276 lines of code.
In contrast, the repositories pertaining to statically-typed programming languages, namely C/C++ and Java, are more complex, featuring an increased count of code files and lines.
For JavaScript, our usage of the Vue.js framework necessitates that models adeptly navigate the framework's templates and development paradigms.
Consequently, JavaScript repositories exhibit the highest number of code files and lines, posing a substantial challenge for LLMs.
Additionally, we have prepared extensive reference acceptance and unit tests for each repository to facilitate rigorous evaluation of the implementation task.


==> src/discussions.tex <==


\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{figures/results_on_language_with_grid.pdf}
    \caption{Performance Break Down on Different Languages. The results are averaged across all repositories and weighted by the number of code lines}
    \label{fig:language_performance}
\end{figure}

\subsection{Model Capacity}
\paragraph{Challenges in Creating C/C++ Makefile and Java Gradle}
The detailed results broken down on different languages are illustrated in Figure~\ref{fig:language_performance}. Makefiles and Gradle files are pivotal in C/C++ and Java repositories, orchestrating file organization, compilation, linking, and managing dependencies. However, models struggle in accurately generating these files. Smaller models often misconstrue the syntax and structure, leading to irrelevant content like misplaced Linux commands or repeating given prompt instructions. Although larger models, such as GPT-4-Turbo, show improvements, they still fall short, exemplified by frequent ``missing separator'' errors in Makefiles. Similarly, Gradle files often lack crucial dependency declarations, a critical oversight leading to Java compilation failures. Another frequent Gradle problem is omitting essential tasks. Although given with necessary ``tests'' and ``acceptanceTests'' prompts, the model often misses these in the Gradle file, but can correct them upon review.

\paragraph{Function Redefinition in Multi-file Repositories}
Models face significant challenges in multi-file repositories contexts, particularly with function redefinitions. Specifically, if a global function is required for the entire repository, it can be defined in any file, and other files just need to correctly reference it. But they tend to redundantly implement the same function across multiple files, suitable for single-file repositories but erroneous in multi-file scenarios. In C/C++, models incorrectly handle header (.h) and implementation (.cpp) files, leading to redundant declarations and conflicting implementations. These issues highlight a gap in the models' understanding of file-specific roles in programming languages.

\paragraph{File Reference and Linkage Errors}
Correct file referencing is essential in multi-file programming repositories. Models, especially those with larger parameters, generally perform well in establishing basic reference logic, such as using ``import'' in Python and ``\#include'' in C++. However, without review, reference errors are common, likely due to the models' sequential code generation approach, which limits their ability to correct earlier mistakes.
More complex reference issues also arise. Models often struggle to differentiate between global functions and class methods, leading to reference errors when attempting to access class methods directly. These errors are challenging to rectify through review. This indicates a need for models to better grasp the intricacies of programming language structures and conventions.

\subsection{Instruction Following}
\paragraph{Naming Errors}
Proper naming in code is crucial for readability and maintainability. Larger models, like GPT-4-Turbo, while capable of generating syntactically correct code, exhibit deficiencies in this area. It inaccurately modifies function and variable names, disrupting the code's functionality. For instance, in ``Graph BFS DFS'', we instruct the use of the ``top()'' method for stack access, yet GPT-4-Turbo incorrectly labels it as ``getTop()''. Furthermore, the model's lack of attention to plurals and capitalization aggravates these errors. Despite reviews, this issue remains inadequately addressed.

\paragraph{Function Parameters and Overloading Errors}
We observe that even some large models, such as GPT-4-Turbo, neglect the correct number of function parameters, missing critical ones. Function overloading is another similar nuanced aspect that many models mishandle. They often overlook the necessity of multiple constructors or methods with varying parameters. For example, in a task like ``area\_calculation'', models fail to create both parameterized and parameterless constructors, focusing solely on the former. This oversight is not significantly rectified in the review stages, as models mistakenly attribute the errors to the test program. They stubbornly resist correcting their generated code, even when provided with clear instructions.

\paragraph{Type Errors}
Models demonstrate a lack of sensitivity to type conversions, especially in strongly-typed languages like C/C++. Errors in matching const types and misusing pointer types are common, and these missteps are not readily resolved in the review process. However, in weakly-typed languages like Python, such issues are less critical but still present a concern for code accuracy.

\paragraph{Variable Scope and Lifecycle Mismanagement}
Models frequently misuse variables beyond their intended scope or lifecycle. For example, they might attempt to use a loop control variable outside its loop. Another issue is the misunderstanding of private and public members in classes, where models inappropriately access private elements from outside the class. This indicates a gap in the models' understanding of encapsulation and scope management in object-oriented programming.

\subsection{Hallucination}
\paragraph{Fabrication of Variables}
A significant challenge is the models' propensity to fabricate non-existent local variables, a problem typically rectified during review. This issue suggests a fundamental limitation in the models' sequential generation process. Unable to retroactively integrate essential variable definitions, the models end up introducing imaginary variables in the code, resulting in apparent inaccuracies.

\paragraph{Misinterpretation of Data Files}
Models also exhibit a tendency to incorrectly interpret data files as Python libraries. They attempt to import methods from these non-existent libraries, leading to further reference errors. This behavior underscores the intricacy involved in handling file references accurately within code generation tasks.

\subsection{Limitations in Testing}
\label{sec:Limitation in test}
% In Acceptance Testing task, we employ an execution-based evaluation method for the generated tests, foregoing manual quality assessments.
% This approach assumes a test is valid if it can accurately assess standard implementation code. However, we observed that smaller models, such as DeepSeek-Coder-6.7B-Instruct, exploit this method.
% They establish arbitrary criteria and invariably provide positive feedback, thereby circumventing a genuine evaluation.
% Larger models like GPT-4-Turbo fell short of our expectations.
% This issue arises because these larger models persistently recall and utilize methods in the original project code, instead of our specially designed versions.
% This tendency originates from a training data bias, where these models are predisposed to original project code, commonly leading to import errors in our evaluation.
In Acceptance Testing task, we employ an execution-based evaluation method for the generated tests, foregoing manual quality assessments. This approach assumes a test is valid if it can accurately assess standard implementation code. However, we observed that smaller models, such as DeepSeek-Coder-6.7B-Instruct, generates meaningless but executable test scripts that do not assert the output of the program but only execute some statement of the project. This can give rise to the statement coverage achieved, but as they do not check the correctness of the output of the function or the program, they cannot really assure the quality of the software system.

Larger models like GPT-4-Turbo fell short of our expectations. They persistently recall and utilize methods in the original repository code, instead of our specially designed versions, leading to frequent import errors. This issue is exemplified in our tests with the ``GeoText'' and ``Stocktrends'' repositories. We modified the original repositories by removing ``\_\_init\_\_.py'' files, expecting models could correctly handle import relationships without them, based on our provided file structures. However, the models continued to follow the import logic of the original repositories, leading to hallucination and inaccurate test generation. This indicates a training data bias, where these models are predisposed to original repository code and show a reluctance to adjust to new circumstance.


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}

